Faster Maximum Inner Product Search in High Dimensions

Maximum Inner Product Search (MIPS) is a ubiquitous task in machine learning applications such as recommendation systems. Given a query vector and $n$ atom vectors in $d$-dimensional space, the goal of MIPS is to find the atom that has the highest inner product with the query vector. Existing MIPS algorithms scale at least as $O(\sqrt{d})$, which becomes computationally prohibitive in high-dimensional settings. In this work, we present BanditMIPS, a novel randomized MIPS algorithm whose complexity is independent of $d$. BanditMIPS estimates the inner product for each atom by subsampling coordinates and adaptively evaluates more coordinates for more promising atoms. The specific adaptive sampling strategy is motivated by multi-armed bandits. We provide theoretical guarantees that BanditMIPS returns the correct answer with high probability, while improving the complexity in $d$ from $O(\sqrt{d})$ to $O(1)$. We also perform experiments on four synthetic and real-world datasets and demonstrate that BanditMIPS outperforms prior state-of-the-art algorithms. For example, in the Movie Lens dataset ($n$=4,000, $d$=6,000), BanditMIPS is 20$\times$ faster than the next best algorithm while returning the same answer. BanditMIPS requires no preprocessing of the data and includes a hyperparameter that practitioners may use to trade off accuracy and runtime. We also propose a variant of our algorithm, named BanditMIPS-$\alpha$, which achieves further speedups by employing non-uniform sampling across coordinates. Finally, we demonstrate how known preprocessing techniques can be used to further accelerate BanditMIPS, and discuss applications to Matching Pursuit and Fourier analysis.

==> 1-abstract.tex <==
% !TEX root = 0-main.tex

\begin{abstract}
Maximum Inner Product Search (MIPS) is a ubiquitous task in machine learning applications such as recommendation systems. 
Given a query vector and $n$ atom vectors in $d$-dimensional space, the goal of MIPS is to find the atom that has the highest inner product with the query vector. 
Existing MIPS algorithms scale at least as $O(\sqrt{d})$, which becomes computationally prohibitive in high-dimensional settings.
% Maximum Inner Product Search (MIPS) is a popular problem in the machine learning literature.
% In high-dimensional settings, however, MIPS queries can become computationally expensive as existing solutions do not scale well with dataset dimensionality.
In this work, we present \algnamenospace, a novel randomized MIPS algorithm whose complexity is independent of $d$. 
\algname estimates the inner product for each atom by subsampling coordinates and adaptively evaluates more coordinates for more promising atoms. The specific adaptive sampling strategy is motivated by multi-armed bandits. 
% We present a state-of-the-art algorithm for MIPS in high dimensions, dubbed \algnamenospace.
% \algname is a randomized algorithm that borrows techniques from multi-armed bandits to reduce the MIPS problem to a best-arm identification problem.
% \algname is more adaptive to the underlying data distribution than previous approaches because its complexity is governed by the average coordinate-wise gap $\Delta$ between the highest and second-highest inner products. When $\Delta$ does not depend on the dataset dimensionality $d$,
% \algname lowers the scaling complexity in $d$ of state-of-the-art algorithms from $O(\sqrt{d})$ to $O(1)$.
We provide theoretical guarantees that \algname returns the correct answer with high probability, while improving the complexity in $d$ from $O(\sqrt{d})$ to $O(1)$. 
%In other words, the runtime of \algname has \textit{no} explicit dependence on the data dimensionality; instead, its runtime is governed by the hardness of the underlying data distribution.
We also perform experiments on four synthetic and real-world datasets and demonstrate that \algname outperforms prior state-of-the-art algorithms. 
For example, in the Movie Lens dataset ($n$=4,000, $d$=6,000), \algname is 20$\times$ faster than the next best algorithm while returning the same answer. 
% We empirically verify the advantages of \algname on several high-dimensional real-world datasets. \algname runs significantly faster than existing approaches and returns the same solution.
\algname requires no preprocessing of the data and includes a hyperparameter that practitioners may use to trade off accuracy and runtime.
We also propose a variant of our algorithm, named \algnamenospace-$\alpha$, which achieves further speedups by employing non-uniform sampling across coordinates. 
Finally, we demonstrate how known preprocessing techniques can be used to further accelerate \algnamenospace, and discuss applications to Matching Pursuit and Fourier analysis. 
\end{abstract}

==> 10-acknowledgements.tex <==
% !TEX root = 0-main.tex

\section{Acknowledgments}



==> unused-toy_example.tex <==
\begin{figure}
\label{fig:toy_problem}
\noindent\resizebox{0.47\textwidth}{!}{\begin{tikzpicture}[cell/.style={rectangle,draw=black},
space/.style={minimum height=1.5em,matrix of nodes,row sep=-\pgflinewidth,column sep=-\pgflinewidth,column 1/.style={font=\ttfamily}},text depth=0.5ex,text height=2ex,nodes in empty cells]
+\matrix (first) [space, column 2/.style={minimum width=3em,nodes={cell,minimum width=3.5em}},column 3/.style={minimum width=3em,nodes={cell,minimum width=3.5em}}, column 4/.style={minimum width=3.5em,nodes={cell,minimum width=3.5em}},row 1/.style={row sep=0.75cm}, ampersand replacement=\&]
{
$q$   \& 1 \& 1 \& \node(a) {1}; \\   $v_1$ \& 1 \& 1 \& 1 \\   $v_2$ \& 0 \& 0 \& \node(c) {0}; \\  $v_3$ \& 0 \& 0 \& 0 \\ $v_4$ \& 0 \& 0 \& 0 \\  };

\matrix (second) [right=of first, space, column 2/.style={minimum width=3em,nodes={cell,minimum width=3.5em}},column 3/.style={nodes={cell,minimum width=3em}}, column 4/.style={minimum width=3.5em,nodes={cell,minimum width=3.5em}},row 1/.style={row sep=0.75cm}, ampersand replacement=\&] at (2,0)
{
   \& \node(b) {1}; \& 1 \& 1 \\  \& 1 \& 1 \& 1 \\  \& \node(d) {0}; \& 0 \& 0 \\  \& 0 \& 0 \& 0 \\ \& 0 \& 0 \& 0 \\  };

\path (a) -- node[auto=false]{\ldots} (b);
\path (c) -- node[auto=false]{\ldots} (d);

\matrix (third) [right=of second, space, column 2/.style={blue, minimum width=3em,nodes={cell,minimum width=3.5em}},column 3/.style={blue, nodes={cell,minimum width=3em}}, column 4/.style={blue, minimum width=3.5em,nodes={cell,minimum width=3.5em}}, cell/.append style={rectangle,draw=blue},row 1/.style={row sep=0.75cm}, ampersand replacement=\&] at (6,0)
{
   \& 1 \& 1 \& \node(e) {1}; \\  \& 1 \& 1 \& 1 \\  \& 0 \& 0 \& \node(g) {0}; \\  \& 0 \& 0 \& 0 \\ \& 0 \& 0 \& 0 \\  };

\matrix (fourth) [right=of third, space, column 2/.style={blue, minimum width=3em,nodes={cell,minimum width=3.5em}},column 3/.style={blue, nodes={cell,minimum width=3em}}, column 4/.style={blue, minimum width=3.5em,nodes={cell,minimum width=3.5em}}, cell/.append style={rectangle,draw=blue},row 1/.style={row sep=0.75cm}, ampersand replacement=\&] at (11,0)
{
   \& \node(f) {1}; \& 1 \& 1 \\  \& 1 \& 1 \& 1 \\  \& \node(h) {0}; \& 0 \& 0 \\  \& 0 \& 0 \& 0 \\ \& 0 \& 0 \& 0 \\  };

\path (e) -- node[auto=false]{\ldots} (f);
\path (g) -- node[auto=false]{\ldots} (h);

\end{tikzpicture}}
\caption{Make this figure bigger. Include (black) and (blue) and that $\Delta = 1$ does not depend on $d$.}
\end{figure}

\martin{I find this toy example too technical. The reader don't need this level of information at this stage of the paper. If you think it's good, maybe move it to later parts, at least after we have talked about the $d$-independent complexity. }
A toy example of MIPS is shown in Figure \ref{fig:toy_problem}.
A reasonable adaptive sampling algorithm should only depend on the average coordinate-wise gap $\Delta$ between the best and second-best atoms' products with the query vector. \martin{$\Delta$ needs definition}
Any such algorithm that is able to determine the highest inner product atom from only the first half of the dimensions need not sample the second half of the dimensions, provided the values in each half are drawn from similar distributions.
At first glance, the problem in Figure \ref{fig:toy_problem} may seem artificially contrived.
However, we demonstrate that many real-world datasets follow a similar structure; we formalize the notion of this structure in Section \ref{sec:theory} and our algorithm in Section \ref{sec:algo}.
